Recursive Backdoors for SAT

A strong backdoor in a formula $\phi$ of propositional logic to a tractable class $\mathcal{C}$ of formulas is a set $B$ of variables of $\phi$ such that every assignment of the variables in $B$ results in a formula from $\mathcal{C}$. Strong backdoors of small size or with a good structure, e.g. with small backdoor treewidth, lead to efficient solutions for the propositional satisfiability problem SAT. In this paper we propose the new notion of recursive backdoors, which is inspired by the observation that in order to solve SAT we can independently recurse into the components that are created by partial assignments of variables. The quality of a recursive backdoor is measured by its recursive backdoor depth. Similar to the concept of backdoor treewidth, recursive backdoors of bounded depth include backdoors of unbounded size that have a certain treelike structure. However, the two concepts are incomparable and our results yield new tractability results for SAT.

==> chapters/abstract.tex <==
\begin{abstract}
    \noindent A backdoor set of a formula of propositional logic is a set of 
    variables such that fixing truth values of the variables from this 
    set results in a formula from a polynomial-time decidable class.
    We introduce and study the concept of \emph{recursive backdoors}, ...
\end{abstract}

==> chapters/prelims/incidence_graphs.tex <==
\textbf{Incidence graphs.} The incidence graph
$\mathrm{inc}(\phi)$ of a formula $\phi$ is a vertex- and edge- colored bipartite
graph. Its vertices are the variables and clauses of $\phi$, colored
with predicates~$V$ and~$C$, respectively, to distinguish variables
and clauses. The edge set of $\mathrm{inc}(\phi)$ is partitioned
into two parts $E_+$ (positive edges) and $E_-$ (negative edges),
where a variable vertex $x$ is connected to a clause vertex $c$ by
an edge $E_\star$ if $x_\star\in \lit(c)$.
We write $G=(V,C,E_+,E_-)$ to denote incidence graphs. Slightly abusing
notation we usually do not distinguish between a formula and its
incidence graph and speak e.g.\ of components of $\phi$ with
implicit reference to the incidence graph of $\phi$.
For an assignment $\tau$ we naturally define
$G[\tau]$ as the incidence graph of $\phi[\tau]$.
If $\tau$ assigns only a single variable
$x \mapsto \star$ we write $G[x_\star]$ for $G[\tau]$.
